Please Don't Go -- Increasing Women's Participation in Open Source Software

Women represent less than 24% of the software development industry and suffer from various types of prejudice and biases. In Open Source Software projects, despite a variety of efforts to increase diversity and multi-gendered participation, women are even more underrepresented (less than 10%). My research focuses on answering the question: How can OSS communities increase women's participation in OSS projects? I will identify the different OSS career pathways, and develop a holistic view of women's motivations to join or leave OSS, along with their definitions of success. Based on this empirical investigation, I will work together with the Linux Foundation to design attraction and retention strategies focused on women. Before and after implementing the strategies, I will conduct empirical studies to evaluate the state of the practice and understand the implications of the strategies.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> Tables/codes.tex <==
\begin{table*}[htb]
\centering
%\scriptsize
\caption{Success meanings from the interviews and the survey classified per Dries et al.'s  model \cite{dries2008career}}
\label{tab:codes}
\footnotesize
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{l|l|l|r|r}
\hline
\rowcolor{gray!35}\multicolumn{2}{c|}{ } & & \multicolumn{1}{|c|}{\textbf{\# Interviews}} & \multicolumn{1}{c}{\textbf{\# Survey }} \\
\rowcolor{gray!35}&\textbf{Region} & \textbf{Participants' IDs (Interviews)}& \multicolumn{1}{c|}{\textbf{(total: 27)}} & \multicolumn{1}{c}{\textbf{(total: 193)}} \\\hline\hline

\multirow{4}{*}{Quad1}
& Cooperation            &  P2, P3, P4, P5, P7, P8, P13, P15, P17, P20, P21 & 11 & 19 \\\cline{2-5}
& Perceived Contribution & P5, P6, P9, P11, P17, P18, P21, P22, P25         & 9  & 57\\ \cline{2-5}
& Recognition            & P1, P9, P13, P22, P23, P25                       & 6  & 29 \\  \cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q1}& \textbf{19} & \textbf{93}\\\hline\hline
 
 
\multirow{4}{*}{Quad2}
& Advancement           & P1, P10, P12, P16, P20, P21, P22, P23, P24 & 8 & 8\\\cline{2-5}
& Performance           & P4                                         & 1 & 0 \\\cline{2-5}
& Factual Contribution  & P2, P6, P12, P14, P18, P19, P20, P21       & 8 & 74\\\cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q2}& \textbf{15} & \textbf{81} \\\hline\hline

\multirow{3}{*}{Quad3}
& Self-Development  & P7, P16, P18, P19, P20, P21, P24 & 7  & 19 \\\cline{2-5}
& Creativity        & P10                              & 1  & 2  \\\cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q3}& \textbf{8} & \textbf{21} \\\hline\hline

 
\multirow{3}{*}{Quad4} 
& Satisfaction  & P1, P5, P10, P16, P21 & 5  & 13 \\ \cline{2-5}
& Security      & P19, P24              & 2  & 17 \\ \cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q4}&  \textbf{7} & \textbf{30} \\\hline\hline

\end{tabular}
}

\resizebox{0.80\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Quad1}: Interpersonal x Affect; \textbf{Quad2}: Interpersonal x Achievement; \textbf{Quad3}: Intrapersonal x Achievement; \textbf{Quad4}: Intrapersonal x Affect\\
The total per quadrant is not the sum of the regions since the participants often provided an answer that was categorized into \textbf{more than one region}.
\end{tabular}
}


\end{table*}

==> Tables/codes_by_role.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\centering
\caption{Quadrants and Regions cited by the Interview's Participants who play roles as coders and non-coders}
\label{tab:codes_by_role}
\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Quadrant}                     & \multirow{2}{*}{Region} & \multicolumn{2}{c|}{Participants ID}            \\ \cline{3-4} 
 &             & Coders (12)               & Non-Coders (15)                \\ \hline
\multirow{2}{*}{Intra-Personal x Affect}      & Satisfaction            & P5, P21                    & P1, P10, P16, P26      \\ \cline{2-4} 
 & Security    & P19, P24             &                           \\ \hline
\multirow{2}{*}{Intra-Personal x Achievement} & Self-Development        & P7, P18, P19, P20, P21, P24 & P12, P16          \\ \cline{2-4} 
 & Creativity  &                      & P10                       \\ \hline
\multirow{3}{*}{Inter-Personal x Affect}      & Perceived Contribution  & P5, P6, P18, P21, P25       & P22, P9, P11, P17 \\ \cline{2-4} 
 & Cooperation & P2, P5, P7, P20, P21 & P3, P4, P8, P13, P15, P17 \\ \cline{2-4} 
 & Recognition & P23, P25, P27             & P1, P9, P13, P22          \\ \hline
\multirow{3}{*}{Inter-Personal x Achievement} & Factual Contribution    & P2, P6, P18, P19, P20, P21  & P12, P14          \\ \cline{2-4} 
 & Advancement & P20, P21, P23, P24, P27   & P1, P10, P16, P22         \\ \cline{2-4} 
 & Performance &                      & P4                        \\ \hline
\end{tabular}
\end{table*}

==> Tables/codes_survey.tex <==
\begin{table*}[htb]
\centering
\caption{Success meanings from the survey classified per Dries et al.'s  model \cite{dries2008career} and per type of contribution, gender and the financial relation with OSS}
\label{tab:codes_survey}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
\hline
  \multicolumn{1}{c}{\multirow{3}{*}{}} &
%  \multirow{3}{*}{\textbf{Region}} &
  &
  \multicolumn{4}{c|}{\textbf{Type of Contribution}} &
  \multicolumn{6}{c|}{\textbf{Gender}} &
  \multicolumn{6}{c|}{\textbf{Employment in OSS}}&
  \multicolumn{2}{c}{}  \\ 
  \cline{3-18} 
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c|}{\textbf{Region}} &
  \multicolumn{2}{c|}{Coders} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Coders\end{tabular}} &
  \multicolumn{2}{c|}{Men} &
  \multicolumn{2}{c|}{Women} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Binary\end{tabular}} &
  \multicolumn{2}{c|}{Paid} &
  \multicolumn{2}{c|}{Unpaid} &
  \multicolumn{2}{c|}{\begin{tabular}[c|]{@{}c@{}}Partially\\Paid\end{tabular}} 
  &
  \multicolumn{2}{c}{\textbf{Total} }\\ \cline{3-20} 
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{}&
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% \\ \hline\hline

\multirow{3}{*}{Quad1} &

Cooperation &
  10 &
  6.1\% &
  5 &
  16.7\% &
  12 &
  7.4\% &
  0 &
  0.0\% &
  2 &
  100.0\% &
  5 &
  13.9\% &
  10 &
  7.3\% &
  0 &
  0.0\% 
    &
  19&
  8.0\%
  \\ \cline{2-20} 

 &

  Perceived Contr. &
  51 &
  26.4\% &
  6 &
  20.0\% &
  52 &
  31.9\% &
  3 &
  18.8\% &
  0 &
  0.0\% &
  11 &
  30.6\% &
  42 &
  30.7\% &
  3 &
  18.8\% 
    &
  57&
  29.5\%
  \\ \cline{2-20} 

 &
  
  Recognition &
  25 &
  15.3\% &
  4 &
  13.3\% &
  24 &
  14.6\% &
  4 &
  25.0\% &
  0 &
  0.0\% &
  5 &
  13.9\% &
  21 &
  15.3\% &
  3 &
  18.8\% 
    &
  29&
  12.1\%
\\ \hline
\multirow{2}{*}{Quad2} &
  Advancement &
  7 &
  4.3\% &
  1 &
  3.3\% &
  7 &
  4.3\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  2 &
  5.6\% &
  4 &
  2.9\% &
  2 &
  12.5\% 
    &
  8&
  4.1\%
  \\ \cline{2-20} 

 &
 
  Performance &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% 
    &
  0&
  0.0\%
  \\ \cline{2-20} 
 
 &
 
  Factual Contr. &
  62 &
  38.0\% &
  12 &
  40.0\% &
  61 &
  37.4\% &
  6 &
  37.5\% &
  1 &
  50.0\% &
  14 &
  38.9\% &
  52 &
  38.0\% &
  6 &
  37.5\% 
    &
  74&
  38.3\%
\\ \hline

\multirow{2}{*}{Quad3} &
  Self-Development &
  15 &
  9.2\% &
  4 &
  13.3\% &
  17 &
  10.3\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  2 &
  5.6\% &
  14 &
  10.2\% &
  2 &
  12.6\% 
  &
  19&
  9.8\%
  \\ \cline{2-20} 
 &
  Creativity &
  1 &
  0.6\% &
  1 &
  3.3\% &
  2 &
  1.2\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  1 &
  2.8\% &
  1 &
  0.7\% &
  0 &
  0.0\% 
    &
  2&
  0.9\%
\\ \hline

\multirow{2}{*}{Quad4} &
  Satisfaction &
  11 &
  6.7\% &
  3 &
  10.0\% &
  11 &
  6.6\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  1 &
  2.8\% &
  11 &
  8.0\% &
  1 &
  6.3\% 
  &
  13&
  5.4\%
  \\ \cline{2-20} 
 &
  Security &
  17 &
  10.4\% &
  0 &
  0.0\% &
  15 &
  9.0\% &
  2 &
  12.5\% &
  0 &
  0.0\% &
  3 &
  8.3\% &
  9 &
  6.6\% &
  5 &
  31.3\% 
  &
  17&
  7.1\%
  \\ \hline


\multicolumn{2}{r|}{Total unique resp.} &
  163 &
   &
  30 &
   &
  165 &
   &
  16 &
   &
  2 &
   &
  36 &
   &
  137 &
   &
  16 &
   & 193
  &
   \\ \hline
\end{tabular}
}

\resizebox{\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Quad1}: Interpersonal x Affect; \textbf{Quad2}: Interpersonal x Achievement; \textbf{Quad3}: Intrapersonal x Achievement; \textbf{Quad4}: Intrapersonal x Affect; \\
The sum of each quadrant can differ from the total of unique respondents as people often provided an answer to the open question that was categorized into more than one region. 
\end{tabular}
}

\end{table*}


==> Tables/demo.tex <==
\begin{table*}[htb]
\centering
\caption{Demographics for the Interview Participants}
\label{tab:demo}
\begin{tabular}{c|l|r|l|l|l}
\hline
\cellcolor{gray!35}\textbf{Participant ID} & \cellcolor{gray!35}\textbf{Gender}        & \cellcolor{gray!35}\textbf{Years in OSS} & \cellcolor{gray!35}\textbf{Main Type of Contribution}  & \cellcolor{gray!35}\textbf{Recruitment} & \cellcolor{gray!35}\textbf{Interview Mode} \\ \hline
P1  & Woman                  & 6 ~~~~~~ & OSS Advocate            & OSCON Speaker & In-person       \\ 
P2  & Woman                  & 5  ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ 
P3  & Woman                  & 13 ~~~~~~ & OSS Treasurer           & OSCON Speaker & In-person       \\ 
P4  & Man                    & 9  ~~~~~~ & OSS System Admin        & OSCON Speaker & In-person       \\ 
P5  & Prefer not to say & 7  ~~~~~~ & OSS Coder               & OSCON Speaker & In-person       \\ 
P6  & Man                    & 5  ~~~~~~ & OSS Coder               & OSCON Speaker & In-person       \\ 
P7  & Man                    & 12 ~~~~~~ & OSS Coder               & OSCON Speaker & In-person       \\ 
P8  & Woman                  & 30 ~~~~~~ & OSS Strategist          & OSCON Speaker & In-person       \\ 
P9  & Man                    & 13 ~~~~~~ & OSS Advocate            & OSCON Speaker & In-person       \\ 
P10 & Woman                  & 20 ~~~~~~ & OSS Advocate            & OSCON Speaker & In-person       \\ 
P11 & Woman                  & 20 ~~~~~~ & OSS Writer              & Snowballing      & Video-conference \\ 
P12 & Woman                  & 20 ~~~~~~ & OSS Advocate and Writer & OSCON Speaker & In-person       \\ 
P13 & Woman                  & 7  ~~~~~~ & OSS Advocate            & Mature project   & Video-conference \\ 
P14 & Woman                  & 20 ~~~~~~ & OSS License Manager     & Mature project   & Video-conference \\ 
P15 & Woman                  & 15 ~~~~~~ & OSS Advocate            & OSCON Speaker    & In-person       \\ 
P16 & Woman                  & 10 ~~~~~~ & OSS Advocate            & Snowballing      & Video conference \\ 
P17 & Woman                  & 5  ~~~~~~ & OSS Project Manager     & OSCON Speaker & In-person       \\ 
P18 & Man                    & 8  ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ 
P19 & Man                    & 8  ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ 
P20 & Man                    & 5  ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ 
P21 & Man                    & 15 ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ 
P22 & Man                    & 10 ~~~~~~ & OSS Advocate            & Mature project   & Video-conference \\ 
P23 & Man                    & 7  ~~~~~~ & OSS Coder               & Snowballing      & Video-conference \\ 
P24 & Man                    & 20 ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ 
P25 & Man                    & 23 ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ 
P26                     & Prefer not to say & 10                    ~~~~~~ & OSS Project Manager & Mature project       & Videoconference         \\ 
P27 & Woman                  & 10 ~~~~~~ & OSS Coder               & Mature project   & Video-conference \\ \hline
\end{tabular}
\end{table*}

==> Tables/demo_old.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\caption{Demographics for the Interview Participants}
\label{tab:demo_old}
\begin{tabular}{|c|c|c|l|}
\hline
\textbf{Participant ID} & \textbf{Gender} & \textbf{Years in OSS} & \textbf{Main Role} \\\hline\hline
P1 & Woman & 6 & OSS Advocate \\\hline
P2 & Woman & 5 & OSS Coder  \\\hline
P3 & Woman & 13 & OSS Treasurer  \\\hline
P4 & Man & 9 & OSS System Admin  \\\hline
P5 & Prefer not to disclose & 7 & OSS Coder  \\\hline
P6 & Man & 5 & OSS Coder  \\\hline
P7 & Man & 12 & OSS Coder  \\\hline
P8 & Woman & 30 & OSS Strategist \\\hline
P9 & Man & 13 & OSS Advocate  \\\hline
P10 & Woman & 20 & OSS Advocate  \\\hline
P11 & Woman & 20 & OSS Writer \\\hline
P12 & Woman & 20 & OSS Advocate and Writer \\\hline
P13 & Woman & 7 & OSS Advocate \\\hline
P14 & Woman & 20 & OSS License Manager \\\hline
P15 & Woman & 15 & OSS Advocate \\\hline
P16 & Woman & 10 & OSS Advocate \\\hline
P17 & Woman & 5 & OSS Project Manager \\\hline
P18 & Man & 8 & OSS Coder \\\hline
P19 & Man & 8 & OSS Coder \\\hline
P20 & Man & 5 & OSS Coder \\\hline
P21 & Man & 15 & OSS Coder \\\hline
P22 & Man & 10 & OSS Advocate \\\hline
P23 & Man & 7 & OSS Coder \\\hline
P24 & Man & 20 & OSS Coder \\\hline
P25 & Man & 23 & OSS Coder \\\hline
P26 & Prefer not to disclose & 10 & OSS Project Manager \\\hline
P27 & Woman & 10 & OSS Coder \\\hline
\end{tabular}
\end{table*}

==> Tables/survey_demo.tex <==
\begin{table}[htb]
\centering
\caption{Demographics for the Survey Respondents}
\label{tab:survey_demo}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|c|ccc|c|c}
\cline{1-3}\cline{5-7}
\cellcolor{gray!35}\textbf{Role} & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}  & \multirow{15}{*}{} & \cellcolor{gray!35}\textbf{Country of Residence} & \cellcolor{gray!35}\textbf{\#} & \cellcolor{gray!35}\textbf{\%}\\\cline{1-3}\cline{5-7}
Coder              & 163 & 84.46\% &                    & Germany              & 89 & 46.11\% \\
Non-Coder          & 30  & 15.54\% &                    & USA                  & 59 & 30.57\% \\\cline{1-3}
\multicolumn{3}{l}{}               &                    & Netherlands          & 12 & 6.22\%  \\\cline{1-3}
\cellcolor{gray!35}\textbf{Gender}             & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}      &                    & Brazil               & 9  & 4.66\%  \\\cline{1-3}
Men                & 165 & 85.49\% &                    & Others               & 23 & 11.92\% \\
Women              & 16  & 8.29\%  &                    & Did not answer       & 1  & 0.52\%  \\\cline{5-7}
Non-Binary         & 2   & 1.04\%  &\multicolumn{1}{l}{}& \multicolumn{3}{l}{}                \\\cline{5-7}
Did not answer     & 10  & 5.18\%  &                    & \cellcolor{gray!35}\textbf{Age}  & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}      \\\cline{1-3}\cline{5-7}
\multicolumn{3}{l}{}               &                    & 24 or less           & 30 & 15.54\% \\\cline{1-3}
\cellcolor{gray!35}\textbf{Financial Relation} & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}       &                    & 25-34                & 60 & 31.09\% \\
Paid               & 36  & 18.65\% &                    & 35-44                & 59 & 30.57\% \\
Unpaid             & 137 & 70.98\% &                    & 45-54                & 27 & 13.99\% \\
Partially Paid     & 16  & 8.29\%  &                    & 55 or more           & 10 & 5.18\%  \\
Did not answer     & 4   & 2.07\%  &                    & Did not answer       & 7  & 3.63\% \\\cline{1-3}\cline{5-7}
\end{tabular}}
\end{table}

==> UnusedText.tex <==
FROM DISCUSSION:

\begin{comment}

%%%EVERYTHING UNTIL \end{comment} IS JUST TO KEEP THE TEXT AROUND
\textbf{========================WIP===============}
To be built:

* Success is multifaceted -- Hard to measure
 
* While different people (non-coder/coder) may follow different bands of the rainbow, the end pot of gold remains the same. Anyways, it is still important to consider diverse meanings. Recognize the contribution with different nature. Be careful with using rankings, badges that focus only on some stuff.

* Both interpersonal and intrapersonal dimensions are important for men, contrary to the existing research. Also: men talked more about subjective things (Cooperation and Perc. contribution) than women, which is interesting because it kind of contradicts past research. Maybe this is because OSS is all about cooperation and community valuing the contribution that we do. Anyways, there is something about OSS that needs to be analyzed in-depth.

\textbf{========================WIP===============}

%\boldification{**People mentioned the success of the community success as being their personal success**}
%Participants also mentioned their personal success as the health of the communities they are part (e.g. \textit{"I think the sign of a healthy open source project is where everybody feels like their voice is heard and their opinion matters"} (P7)), how the contributor perceives themselves in a community \textit{"success is... the way that I can help"}, and how the external world perceives their contributions (e.g., \textit{"impact on people in the world"} (P11). 

%\textit{"making sure that people feel heard, that you're able to unwind it"} (P3)), how the success of the project may reflect on their success %being able to bring health to the project they are working for (e.g. . Some participants mentioned that community and project success can also represent personal success for them (e.g. \textit{"success is... the way that I can help"} (P3) or \textit{"I think having a healthy community is probably the most important thing"} (P4)). The mixing concepts continued when  participants mentioned the success of other people can also be a way to achieve their goals and own personal success (e.g. \textit{"The code is usually the easy part, but making sure you have systems and processes in place for people to be successful, and to help you meet your goals"} (P4)). 

\noindent\textbf{Success is a dynamic and multifaceted concept.} We found that some concepts related to success represent different meanings for different people. Money is an example. Money represents \textsc{Security} when participants said success is when they can live from OSS. Money represents \textsc{Advancement} when participants mentioned having a career growth as their salary goes up (P16, P21). Another example, when recognition was mentioned by participants as contributing for a recognized community (P20, P21), it represents \textsc{Advancement}, or progressing in the career. When recognition was mentioned as being their own names well-known or having notoriety (P1, P9, P13, P23, P25 and P27), it represents \textsc{Recognition}. 
%Indeed, recognition plays a relevant part on OSS contributors' motivations \cite{ghosh2005understanding,harsworking,hertel2003motivation,von2012carrots}.

\boldification{**Measuring subjective concepts of career success is hard.} 
\noindent\textbf{Success of OSS contributors can take many forms and be challenging to measure.} The non-technical types of contributions, which are becoming more common~\cite{trinkenreich2020pathways} and can have subjective meanings --\textit{Many times it is easier to set up a metric that measures the quantitative thing, but things like outreach, mentoring, inclusion work, and documentation is, it is harder to measure that with quantitative things, and have impact.'' (P11)}. This indicates that the concept of success may include subjective perspectives, and be challenging to measure.

\boldification{**Previous works about measuring success in OSS only looked at the project/community's success, and can be used for some definitions from Intrapersonal dimension}
Career measures for subjective definitions, as for example Satisfaction~\cite{greenhaus1990effects}, have been criticized for not including all possible dimensions people may use to define and evaluate career success~\cite{arthur2005career,heslin2005conceptualizing}. However, even if it were feasible to have a list of all possible criteria used by people to evaluate career success, transforming this knowledge into a workable measure of career success would still remain challenging~\cite{dries2008career}.  Research in OSS devised metrics to evaluate the project or product success (e.g.  \cite{crowston2003defining,  subramaniam2009determinants, piggot2013healthy} and code-centric contributions (e.g. number of source code contributions submitted and accepted by the project) \cite{roberts2006understanding}, but not the achievement of aspects related to individual success.

\boldification{***Contributions can bring Recognition and more}
\textbf{Contributions can bring \textsc{Recognition} and both can be ways to achieve other interests.} The reason behind why OSS contributors make \textsc{Factual Contribution} and seek outreach (\textsc{Perceived Contribution}) can be related to pure altruism of producing value to others (e.g. \textit{``Getting other people inspired for the concept/idea"} - S122; or can be related to other interests. According to P9, the impact your project bring can cause \textsc{Recognition}, because when producing \textit{``something used by others, or useful to others, you get some recognition, you are creating community, people you do networking''}. The person can seek outreach in order to achieve a goal to sell products built upon OSS (\textit{
``I want outreach for people to recognize the brand, to recognize me as gear... because that makes my life easier, makes selling services easier because I don't have to educate as much"} - P22). Even using the word ``recognition", the reasoning for achieving outreach was to facilitate selling OSS services, which is part of Factual Contribution region. Outreach can also be a success meaning related to recognition, when the person mentions having fame (\textit{``Famous. Creator of a well known project. The project has to be useful for many others"} - S010) or notoriety (\textit{``A one left their mark on a good project"} - S057). Contributions to the project can bring \textsc{Recognition} by having your name well-known and also \textsc{Advancement} as receiving job opportunities (e.g. \textit{``A software engineer makes contributions and can put that on his resume as a reference. If he (sic) is well evaluated for this in the market, this is success."} (P19)). When \textsc{Factual Contributions} are motivated by self-marketing, it may help to lure the best programmers and most productive minds away from the project into more profitable ones˜\cite{harsworking}. Motivations and success perceptions need to be aligned to retain professionals.


\boldification{***Coders and non-coders had similar perceptions of success on Factual/Perceived Contribution and Recognition. However, only coders cited Security, and more non-coders mentioned Cooperation}
\textbf{Coders and non-coders from our sample perceive success in similar ways, with some imbalance, though.}
\textsc{Factual Contribution}, \textsc{Perceived Contribution}, and \textsc{Recognition} was very similar for all contributors. While we noticed that more coders mentioned success aspects related to \textsc{Security}, more non-coders mentioned \textsc{Cooperation}. The current code-centricity perspective of OSS projects is limited. When stereotyping OSS projects as communities of developers, we neglect the set non-code related tasks and all the relevant contribution types without which a project could not be what it is~\cite{carillo2015many, trinkenreich2020pathways}. Non-code contributors are frequently excluded from analysis of OSS communities. OSS projects strongly depend on the well-being of OSS communities which is, in-turn, closely tied to both coders and non-coders, who help care, sustain, and protect communities~\cite{carillo2017makes}. Emphasis on code contributions within OSS communities may devalue other types of contributions~\cite{barcomb2020managing}. Coders are commonly thankful for having their names in a ``credits" file, but non-coder are commonly overlooked~\cite{barcomb2018uncovering}. The literature presents several techniques based on code-related metrics to evaluate a coder contributor work and expertise, as their activity in Stack Overflow and GitHub~\cite{huang2016cpdscorer} and their performance on a set of programming tasks~\cite{bergersen2014construction}. Having non-coders mentioning \textsc{Recognition} as an meaning of success, may indicate that it they are claiming for ways to  get appropriate ``credit" for their work, measure and expose their expertise.

\boldification{***Non-coders cited more community-centric than coders***}
\textbf{Non-coders from our sample mentioned more success meanings related to community-centric than coders}. In our study, this region represented the community-centered and collaborative side of OSS. This was an expected result, since many non-coders play community management activities (e.g. advocate, strategist, treasurer), which include ensuring that community members can work productively and that newcomers can easily join the project and also to shape, maintain, monitor and report the pulse of the community~\cite{michlmayr2009community, maenpaa2017many}. However, even in a lower rate than non-coders, having 10 coders considering success as being able to support the community to grow and succeed showed that coders encompass a situated profile of hybrid contributors~\cite{barcellini2014situated,wang2020unveiling}, and they are not solitary hackers anymore. Indeed, performance-related behavior goes well beyond the common idea that contributing to an OSS project is only about writing code. There are three overall types of citizenship-like behavior that can benefit a community: behavior related to help the individuals, to help the software project, and to help the overall community~\cite{carillo2017makes}.
%The performance of a contributor can be associated to the functioning and sustainability of a given community even though their code contribution is limited or even non-existent~\cite{carillo2017makes}.
%The importance that OSS contributors give to the community-centered view is aligned with the notion that a person is good for the community when having the social ability to contribute to the well-being of the community.


\boldification{**Men cited more Cooperation and Perceived Contribution, which are regions from Affect dimension. However, in previous works, men only considered tangible aspects of success**}
%\textbf{We found that men in our sample value more the objective and %Women cited more success meanings related to \textsc{Satisfaction} than men, and men cited more success meanings related to \textsc{Security} than women (see Table \ref{tab:codes_survey}. 
Success meanings related to \textsc{Cooperation} and \textsc{Perceived Contribution} regions, that are part of the Affect end (i.e. subjective side, feelings and perceptions), were more cited by men than women. This is opposite to what Dyke el. al~\cite{dyke2006we}, Cho et. al~\cite{cho2017south} and Anne Marie Porter~\cite{porter2019physics} presented that for men, success is related to tangible and objective outcomes. Men from our sample also talked about their feelings and showed they can also value subjective accomplishments for being successful.
%Dyke el. al~\cite{dyke2006we} presented how women and men define success. For women, success was associated to a personal idea of balance and to the relationships; and for men, success is more material, associated to money and earnings. Our results was also opposite to what Cho et. al~\cite{cho2017south} found about how Korean executives differ in terms of gender when defining being successful. The majority of men executives mentioned success as tangible and objective outcomes, including achievements, recognition, reputation, positions and promotion, while all women executives mentioned more subjective meanings for success, as  work–life balance, feeling happy, respect from family, relationships and personal growth. Moreover, another similar finding was reported by Anne Marie Porter~\cite{porter2019physics}, who reported that men usually attributed career success to skills and abilities, and women to social support. 

%Moreover, having 6\% (10 out of 165) of the mentioning success for them is about being happy or part of the scene (\textsc{Satisfaction}) was a surprise. So, men can also be susceptible on talking about their feelings and can also need subjective accomplishments for being successful.

%\boldification{**New regions for the model}
%\textbf{Motivation is a candidate new region for the model.} Finally, although we observed happiness when P1 mentioned that success is \textit{"having a job that I want to wake up for every day"}, we found it also connected to a motivation aspect, which may have a different understanding compared to satisfaction, according to Software Engineering literature~\cite{francca2014motivated}. As a future work, we plan to evaluate an extension for the model, which could include a \textsc{Motivation} region.
\end{comment}
